HNLB: Utilizing Hardware Matching Capabilities of NICs for Offloading Stateful Load Balancers

In order to scale web or other services, the load on single instances of the respective service has to be balanced. Many services are stateful such that packets belonging to the same connection must be delivered to the same instance. This requires stateful load balancers which are mostly implemented in software. On the one hand, modern packet processing frameworks supporting software load balancers, such as the Data Plane Development Kit (DPDK), deliver high performance compared to older approaches. On the other hand, common Network Interface Cards (NICs) provide additional matching capabilities that can be utilized for increasing the performance even further and in turn reduce the necessary server resources. In fact, offloading the packet matching to hardware can free up CPU cycles of the servers. Therefore, in this work, we propose the Hybrid NIC-offloading Load Balancer (HNLB), a high performance hybrid hardware-software load balancer, utilizing the NIC-offloading hardware matching capabilities. The results of our performance evaluations show that the throughput using NIC offloading can be increased by up to 50%, compared to a high performance software-only implementation. Furthermore, we investigated the limitations of our proposed approach, e.g., the limited number of possible concurrent connections.

==> content/05_methodology.tex <==
\section{Methodology}

Here we could put the simulation
